AirLetters: An Open Video Dataset of Characters Drawn in the Air

We introduce AirLetters, a new video dataset consisting of real-world videos of human-generated, articulated motions. Specifically, our dataset requires a vision model to predict letters that humans draw in the air. Unlike existing video datasets, accurate classification predictions for AirLetters rely critically on discerning motion patterns and on integrating long-range information in the video over time. An extensive evaluation of state-of-the-art image and video understanding models on AirLetters shows that these methods perform poorly and fall far behind a human baseline. Our work shows that, despite recent progress in end-to-end video understanding, accurate representations of complex articulated motions -- a task that is trivial for humans -- remains an open problem for end-to-end learning.

==> figures/hist.tex <==
\begin{figure}[tb]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=.5\textwidth]{figures/assets/duration_hist.pdf} & \includegraphics[width=.495\textwidth]{figures/assets/fps_hist.pdf}
        % \multicolumn{2}{c}{\includegraphics[width=\textwidth]{figures/assets/classes_hist.pdf}}
        % \includegraphics[width=.5\textwidth]{figures/assets/hw_hist.pdf} & \includegraphics[width=.5\textwidth]{figures/assets/frames_hist.pdf}
    \end{tabular}
    \caption{\textbf{Distribution of Videos.} We show histograms visualizing the distribution of (a) video durations, and (b) FPS of videos.}
    % (c) the number of videos per class where $\mathcal{N}$ represents the class ``doing nothing'' and $\mathcal{O}$ represents the class ``doing something else''}
    \label{fig:novideos}
\end{figure}
